Has Your Pretrained Model Improved? A Multi-head Posterior Based Approach

The emergence of pre-trained models has significantly impacted Natural Language Processing (NLP) and Computer Vision to relational datasets. Traditionally, these models are assessed through fine-tuned downstream tasks. However, this raises the question of how to evaluate these models more efficiently and more effectively. In this study, we explore a novel approach where we leverage the meta-features associated with each entity as a source of worldly knowledge and employ entity representations from the models. We propose using the consistency between these representations and the meta-features as a metric for evaluating pre-trained models. Our method's effectiveness is demonstrated across various domains, including models with relational datasets, large language models and image models.

==> fig/CLIPModelsBasic/CLIPAnalysisBreedsMLEvsLP.tex <==
\section{Analysis of CLIP Embeddings on the BREEDS hierarchy}
\label{ssec:CLIPBreedsPerRegPerNetPerData}

\subsection{Models} 
\label{sssec:CLIPModelsPerRegPerNetPerData}
For the purpose of this study we use CLIP-ViT transformers ViT-L/14, ViT-B/32, ViT-B/16 trained on 224 px $\times$ 224 px images as image encoders. Where ViT-L/14 encodes each image into a 768 dimensional embedding and ViT-B/16 and ViT-B/32 encode each image as a 512 dimensional embedding. \\

\subsection{BREEDS Datasets}
\label{ssec:breedsdatasetPerRegPerNetPerData}

\subsection{Experimental Analysis}
\label{ssec:CLIPBreedsAnalysisPerRegPerNetPerData}



\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.32\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelsBreeds/Figures_l2_1e-6/entity13/metrics-entity13-ViT-B-16.pdf}
            \caption{CLIP ViT-B-16 on entity13}
            \label{fig:entity13-vitb16}
        \end{subfigure}
        \begin{subfigure}{0.32\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelsBreeds/Figures_l2_1e-6/entity13/metrics-entity13-ViT-B-32.pdf}
            \caption{CLIP ViT-B-32 on entity13}
            \label{fig:entity13-vitb32}
        \end{subfigure}
        \begin{subfigure}{0.32\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelsBreeds/Figures_l2_1e-6/entity13/metrics-entity13-ViT-L-14.pdf}
            \caption{CLIP ViT-L-14 on entity13}
            \label{fig:entity13-vitl14}
        \end{subfigure}
    \end{center}
    \caption{Layerwise CLIP Embedding Posterior Analysis. In this figure we provide analysis the layerwise behaviour of our metric's value, shown with purple lines in the bottom plot, with that of a linear probe, shown with blue lines on the top plots. We do this for ViT-B/16,ViT-B/32 and ViT-L/14 CLIP models on the enity13 dataset of the BREEDS hierarchy. The training set characteristics are denoted by a solid line and the validation set by a dashed line.}
    \label{fig:CLIPposteriorAnalysisBreeds-entity13}
\end{figure}



==> fig/CLIPModelsBasic/CLIPAnalysisBreedsMLEvsLPallNetPerReg.tex <==
\section*{Appendix}
\section{Fixed regularization cross Model analysis of CLIP Embeddings on the BREEDS hierarchy}
\label{sec:CLIPBreedsallNetPerRegPerData}

In this section we demonstrate supplementary results to the finding shown in \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_demo} regarding the dissonance between linear probe accuracies and log posterior values over the performance of some layers in the CLIP models. \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperrege30} demonstrates the findings for entity 30, \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperregl17} for living 17 and \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperregnl26} for non living 26.




\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/entity30/metrics-entity30-uncorr.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 30 breeds dataset. Class covariance matrix assumes uncorrelated embedding dimensions, thereby just using the diagonal of the covariance matrix.}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege30_diag}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/entity30/metrics-entity30-0.001.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 30 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-3}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege30_1e-3_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/entity30/metrics-entity30-1e-06.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 30 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-6}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege30_1e-6_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/entity30/metrics-entity30-1e-09.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 30 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-9}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege30_1e-9_demo}
        \end{subfigure}
    \end{center}
    \caption{Layerwise multi model analysis of log posterior performance with linear probe performance for a given regularization parameter over entity 30 Breeds Dataset.}
    \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege30}
\end{figure}



\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/living17/metrics-living17-uncorr.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for living 17 breeds dataset. Class covariance matrix assumes uncorrelated embedding dimensions, thereby just using the diagonal of the covariance matrix.}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperregl17_diag}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/living17/metrics-living17-0.001.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for living 17 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-3}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperregl17_1e-3_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/living17/metrics-living17-1e-06.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for living 17 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-6}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperregl17_1e-6_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/living17/metrics-living17-1e-09.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for living 17 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-9}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperregl17_1e-9_demo}
        \end{subfigure}
    \end{center}
    \caption{Layerwise multi model analysis of log posterior performance with linear probe performance for a given regularization parameter over living 17 Breeds Dataset.}
    \label{fig:CLIPposteriorAnalysisBreeds-allnetperregl17}
\end{figure}



\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/nonliving26/metrics-nonliving26-uncorr.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for non living 26 breeds dataset. Class covariance matrix assumes uncorrelated embedding dimensions, thereby just using the diagonal of the covariance matrix.}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperregnl26_diag}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/nonliving26/metrics-nonliving26-0.001.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for non living 26 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-3}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperregnl26_1e-3_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/nonliving26/metrics-nonliving26-1e-06.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for non living 26 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-6}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperregnl26_1e-6_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/nonliving26/metrics-nonliving26-1e-09.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 13 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-9}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperregnl26_1e-9_demo}
        \end{subfigure}
    \end{center}
    \caption{Layerwise multi model analysis of log posterior performance with linear probe performance for a given regularization parameter over non living 26 Breeds Dataset.}
    \label{fig:CLIPposteriorAnalysisBreeds-allnetperregnl26}
\end{figure}





==> fig/CLIPModelsBasic/CLIPAnalysisBreedsMLEvsLPperNetAllReg.tex <==
\section{Fixed Network cross regularization analysis of CLIP Embeddings on the BREEDS hierarchy}
\label{ssec:CLIPBreedsPerNetAllRegPerData}

In this section


\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/entity13/metrics-entity13-ViT-B-16.pdf}
            \caption{}
            \label{}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/entity13/metrics-entity13-ViT-B-32.pdf}
            \caption{}
            \label{}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/entity13/metrics-entity13-ViT-L-14.pdf}
            \caption{}
            \label{}
        \end{subfigure}
    \end{center}
    \caption{}
    \label{fig:CLIPposteriorAnalysisBreeds-pernetallrege13}
\end{figure}




\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/entity30/metrics-entity30-ViT-B-16.pdf}
            \caption{}
            \label{}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/entity30/metrics-entity30-ViT-B-32.pdf}
            \caption{}
            \label{}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/entity30/metrics-entity30-ViT-L-14.pdf}
            \caption{}
            \label{}
        \end{subfigure}
    \end{center}
    \caption{}
    \label{fig:CLIPposteriorAnalysisBreeds-pernetallrege30}
\end{figure}



\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/living17/metrics-living17-ViT-B-16.pdf}
            \caption{}
            \label{}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/living17/metrics-living17-ViT-B-32.pdf}
            \caption{}
            \label{}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/living17/metrics-living17-ViT-L-14.pdf}
            \caption{}
            \label{}
        \end{subfigure}
    \end{center}
    \caption{}
    \label{fig:CLIPposteriorAnalysisBreeds-pernetallregl17}
\end{figure}




\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/nonliving26/metrics-nonliving26-ViT-B-16.pdf}
            \caption{}
            \label{}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/nonliving26/metrics-nonliving26-ViT-B-32.pdf}
            \caption{}
            \label{}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsPerNetAllRegPerDataset/nonliving26/metrics-nonliving26-ViT-L-14.pdf}
            \caption{}
            \label{}
        \end{subfigure}
    \end{center}
    \caption{}
    \label{fig:CLIPposteriorAnalysisBreeds-pernetallregnl26}
\end{figure}

==> fig/CLIPModelsBasic/CLIPAnalysisBreedsMLEvsLPtotal.tex <==
\section{Experiment analysis of CLIP Embeddings on the BREEDS hierarchy}
\label{ssec:CLIPBreedsPerData}
In this section we assess the ability of our metric to predict the classification performance on embeddings of 3 pretrained CLIP \citep{radford2021learning} models on 4 datasets from the Breeds Hierarchy \citep{santurkar2020breeds}, namely entity 13, entity 30, living 17 and non living 26.

\subsection{Models} 
\label{sssec:CLIPModelserData}
For the purpose of this study we use CLIP-ViT transformers ViT-L/14, ViT-B/32, ViT-B/16 trained on 224 px $\times$ 224 px images as image encoders, where ViT-L/14 encodes each image into a 768 dimensional embedding and ViT-B/16 and ViT-B/32 encode each image as a 512 dimensional embedding.
For each of the networks we obtained model embeddings for the final image encoder as well as the mean embeddings of internal Multi-Head Self Attention Layers. We train a linear probe on the ImageNet \citep{5206848} training subset of the Breeds dataset as well learn the parameters for estimating the MAP. We then correlate the performance of these 2 metrics to better understand the behaviour of our trained posterior and present the results in \autoref{fig:CLIPposteriorAnalysisBreeds-allnetallregalldatasets}.

\subsection{Experimental Analysis}
\label{ssec:CLIPBreedsAnalysisPerData}

\begin{table*}[!htb]
    \begin{minipage}{.5\linewidth}
        \centering
        \setlength{\tabcolsep}{4.5pt}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
        \hline 
        \multicolumn{7}{|c|}{Entity 13} \\
        \hline
        Data $\rightarrow$ & \multicolumn{3}{|c|}{Train Set} & \multicolumn{3}{|c|}{Val. Set}\\
        \hline
        Reg. $\downarrow$  & B16 & B32 & L14 & B16 & B32 & L14\\
        \hline
        $Diag$ &  .99  & .99  & .98  & .99 & .99 & .97 \\
        \hline
        $10^{-3}$ & .97  & .99  & .97  & .97 & .98  & .95 \\
        \hline
        $10^{-6}$ & .97 & .96 & .98 & .99  & .98  & .99 \\
        \hline
        $10^{-9}$ & .96  & .95  & .98 & .99  & .99  & .99 \\
        \hline
        \end{tabular}
    \caption{In this table we show the Pearson's Correlation between layerwise MAP computed over various regularizations and layerwise linear probe accuracy for \autoref{fig:entity13-allnetallreg} on the training and validation sets of entity 13 dataset of the Breeds Hierarchy.}
    \label{tab:entity13pearcorr}
    \end{minipage}
    \hspace{5mm}
    \begin{minipage}{.5\linewidth}
        \centering
        \setlength{\tabcolsep}{4.5pt}
         \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
            \hline 
            \multicolumn{7}{|c|}{Entity 30} \\
            \hline
            Data $\rightarrow$ & \multicolumn{3}{|c|}{Train Set} & \multicolumn{3}{|c|}{Val. Set}\\
            \hline
            Reg. $\downarrow$  & B16 & B32 & L14 & B16 & B32 & L14\\
            \hline
            $Diag$ & .99  & .99  & .99 & .99 & .99 & .98 \\
            \hline
            $10^{-3}$ & .98  & .97  & .98  & .98 & .98  & .98 \\
            \hline
            $10^{-6}$ & .85  & .83  & .89 & .97 & .96 & .99 \\
            \hline
            $10^{-9}$ & .8  &  .76 & .87 & .96 & .96 & .98 \\
            \hline
        \end{tabular}
        \caption{Pearson's Correlation between layerwise MAP computed over various regularizations and layerwise linear probe accuracy for \autoref{fig:entity30-allnetallreg} on the training and validation sets of entity 30 dataset of the Breeds Hierarchy.}
    \label{tab:entity30pearcorr}
    \end{minipage}
    \vspace{5mm}
    \begin{minipage}{.5\linewidth}
        \centering
        \setlength{\tabcolsep}{4.5pt}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
        \hline 
        \multicolumn{7}{|c|}{Living 17} \\
        \hline
        Data $\rightarrow$ & \multicolumn{3}{|c|}{Train Set} & \multicolumn{3}{|c|}{Val. Set}\\
        \hline
        Reg. $\downarrow$  & B16 & B32 & L14 & B16 & B32 & L14\\
        \hline
        $Diag$ & .99  & .99  & .99  & .99 & .99  & .98 \\
        \hline
        $10^{-3}$ & .93  & .93  & .95 & .97 & .96 & .99  \\
        \hline
        $10^{-6}$ & .68  & .65  & .72  & .93 & .94 & .97 \\
        \hline
        $10^{-9}$ & .57  & .49  & .64 & .93 & .95 & .97 \\
        \hline
        \end{tabular}
        \caption{Pearson's Correlation between layerwise MAP computed over various regularizations and layerwise linear probe accuracy for \autoref{fig:living17-allnetallreg} on the training and validation sets of living 17 dataset of the Breeds Hierarchy.}
    \label{tab:living17pearcorr}
    \end{minipage}%
    \hspace{5mm}
    \begin{minipage}{.5\linewidth}
        \centering
        \setlength{\tabcolsep}{4.5pt}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
        \hline 
        \multicolumn{7}{|c|}{Non Living 26} \\
        \hline
        Data $\rightarrow$ & \multicolumn{3}{|c|}{Train Set} & \multicolumn{3}{|c|}{Val. Set}\\
        \hline
        Reg. $\downarrow$  & B16 & B32 & L14 & B16 & B32 & L14\\
        \hline
        $Diag$ &  .99 & .99  & .98 & .99  & .99 & .98 \\
        \hline
        $10^{-3}$ & .98  & .95  & .98 & .98  & .98 & .97 \\
        \hline
        $10^{-6}$ & .72  & .67  & .75 & .97 & .97 & .99 \\
        \hline
        $10^{-9}$ & .54  & .42  & .64 & .96 & .97 & .98 \\
        \hline
        \end{tabular}
        \caption{Pearson's Correlation between layerwise MAP computed over various regularizations and layerwise linear probe accuracy for \autoref{fig:nonliving26-allnetallreg} on the training and validation sets of non living 26 dataset of the Breeds Hierarchy.}
    \label{tab:nonliving26pearcorr}
    \end{minipage}
\end{table*}



For the purpose of this study we measure the correlation between MAP and linear probe accuracies learned and computed over the embeddings of the training set and validation set. The results for which are shown in \autoref{tab:entity13pearcorr}, \autoref{tab:entity30pearcorr},\autoref{tab:living17pearcorr} and \autoref{tab:nonliving26pearcorr} for \autoref{fig:entity13-allnetallreg}, \autoref{fig:entity30-allnetallreg}, \autoref{fig:living17-allnetallreg} and \autoref{fig:nonliving26-allnetallreg} respectively. In \autoref{fig:CLIPposteriorAnalysisBreeds-allnetallregalldatasets} we demonstrate the on a macro level both MAP and linear probe performance correlate. This is across various settings of regularizations for our learned metric over various Breeds Datasets and CLIP Models.





\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetAllRegPerDataset/entity13/metrics-entity13.pdf}
            \caption{CLIP Models analyzed with multiple regularizations - entity13. The pearson correlations between layerwise MAPs for various regularizations and layerwise linear probe accuracies is shown in \autoref{tab:entity13pearcorr}.}
            \label{fig:entity13-allnetallreg}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetAllRegPerDataset/entity30/metrics-entity30.pdf}
            \caption{CLIP Models analyzed with multiple regularizations - entity30. The pearson correlations between layerwise MAPs for various regularizations and layerwise linear probe accuracies is shown in \autoref{tab:entity30pearcorr}}
            \label{fig:entity30-allnetallreg}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetAllRegPerDataset/living17/metrics-living17.pdf}
            \caption{CLIP Models analyzed with multiple regularizations - living17. The pearson correlations between layerwise MAPs for various regularizations and layerwise linear probe accuracies is shown in \autoref{tab:living17pearcorr}}
            \label{fig:living17-allnetallreg}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetAllRegPerDataset/nonliving26/metrics-nonliving26.pdf}
            \caption{CLIP Models analyzed with multiple regularizations - nonliving26. The pearson correlations between layerwise MAPs for various regularizations and layerwise linear probe accuracies is shown in \autoref{tab:nonliving26pearcorr}}
            \label{fig:nonliving26-allnetallreg}
        \end{subfigure}
    \end{center}
    \caption{In this figure we present the evolution of layerwise MAP and linear probe accuracies for all CLIP Models on all datasets across varying regularizations strengths to demonstrate correlations between MAP and linear probe performance. The quantitative results for each settings are shown from \autoref{tab:entity13pearcorr}-\autoref{tab:nonliving26pearcorr}.}
    \label{fig:CLIPposteriorAnalysisBreeds-allnetallregalldatasets}
\end{figure}


However despite this correlation, the metric is not a reliable indicator of embedding performance as many a times it can predict lower values for models which have higher linear separability as indicated by the linear probe accuracy for the embedding of that given layer, we show one such counter study in \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_demo} with additional results available in \autoref{sec:CLIPBreedsallNetPerRegPerData}. In \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_diag_demo} for a MAP model which assumes uncorrelated dimensions we observe that for many earlier and later layers of the CLIP models, the order of performance predicted by log posterior isn't the same as one predict by linear probes on the embedding of that layer. This is particularly evident in case of ViT-L/14 model at both the initial and final layers of the network. A similar phenomena is also observed in \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_1e-3_demo}, which imposes a higher regularization on the class covariance matrix learned to estimate the posterior. But this issue doesn't completely resolve, although is less severe, when reducing the regularization on the learned class covariance as shown in \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_1e-6_demo} and \autoref{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_1e-9_demo} for regularizations $10^{-6}$ and $10^{-9}$ respectively.


\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/entity13/metrics-entity13-uncorr.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 13 breeds dataset. Class covariance matrix assumes uncorrelated embedding dimensions, thereby just using the diagonal of the covariance matrix.}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_diag_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/entity13/metrics-entity13-0.001.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 13 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-3}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_1e-3_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/entity13/metrics-entity13-1e-06.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 13 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-6}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_1e-6_demo}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/CLIPModelBreedsAllNetPerRegPerDataset/entity13/metrics-entity13-1e-09.pdf}
            \caption{Layerwise MAP (Log. Posterior) value vs layerwise linear probe value for entity 13 breeds dataset. The regularization used to learn the class covariance matrix was $10^{-9}$}
            \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_1e-9_demo}
        \end{subfigure}
    \end{center}
    \caption{Layerwise multi model analysis of log posterior performance with linear probe performance for a given regularization parameter over entity 13 Breeds Dataset.}
    \label{fig:CLIPposteriorAnalysisBreeds-allnetperrege13_demo}
\end{figure}




\subsection{BREEDS Datasets}
\label{ssec:breedsdatasetPerData}
Breeds Hierarchy \citep{santurkar2020breeds} was by leveraging and modifying the WordNet \citep{miller-1994-wordnet} hierarchy for the ImageNet \citep{5206848} dataset to group together semantically similar classes into 1 superclass. The original purpose of creating this hierarchy was to use the subpopulations present in superclasses to detect a model's robustness to distribution shift but for the purpose of this study we leverage the entire datasets to evaluate the performance of our metric in predicting generalization of CLIP models on those embeddings.



==> fig/CLIPModelsBasic/CLIPAnalysisImageNetSuperClass.tex <==
\section{Analysis of CLIP Embeddings for ImageNet Subsets}
\label{ssec:CLIPRobustness}
In this section we continue the analysis on CLIP Image Encoder \citep{radford2021learning} embeddings on subsets of ImageNet based on superclass as defined by the Robustness library \citep{robustness,engstrom2019adversarial,santurkar2019image,santurkar2020breeds}. The experimental setup is explained next.\\

\subsection{Datasets}
\label{sssec:robustnessDatasets}
To Test our approach we use 5 ImageNet\citep{5206848} subsets using superclass labels based on WordNet\citep{miller-1994-wordnet} hierarchy from the robustness benchmarks \citep{robustness,engstrom2019adversarial,santurkar2019image,santurkar2020breeds}. The datasets are namely: big-12, geirhos-16, living-9, mixed-10, mixed-13. The dataset size statistics are included in \autoref{tab:robustnessStatsImageNetSuperClasses} and the dataset label composition in \autoref{tab:DataSetComp}.\\

% Dataset Stats

\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{ Dataset Statistics of Robustness ImageNet Superclasses}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Training Samples & 308494 & 40517 & 92632 & 77237 & 100233 \\
            \hline
            Testing Samples & 12005 & 1600 & 3603 & 3000 & 3903 \\
            \hline
            Classes & 12 & 16 & 9 & 10 & 13\\
            \hline
        \end{tabular}
    \end{center}
    \caption{Dataset Statistics}
    \label{tab:robustnessStatsImageNetSuperClasses}
\end{table}

% Dataset composition table

\begin{table}[ht] 	
	\begin{center}
    	\begin{tabular}{|c|p{11cm}|}
    		% \multicolumn{2} {Dataset composition }
                \hline Dataset  & Class Composition \\
    		\hline  big-12  & Dog (n02084071), Structure (n04341686),
                    Bird (n01503061), Clothing (n03051540),
                    Vehicle(n04576211), Reptile (n01661091),
                    Carnivore (n02075296), Insect (n02159955),
                    Instrument (n03800933), Food (n07555863),
                    Furniture (n03405725), Primate (n02469914)\\
    		\hline  geirhos-16  & Aircraft (n02686568), Bear (n02131653),
                    Bicycle (n02834778), Bird (n01503061),
                    Boat (n02858304), Bottle (n02876657),
                    Car (n02958343), Cat (n02121808),
                    Char (n03001627), Clock (n03046257),
                    Dog (n02084071), Elephant (n02503517),
                    Keyboard (n03614532), Knife (n03623556),
                    Oven (n03862676), Truck (n04490091)\\
    		\hline  living-9  & Dog (n02084071), Bird (n01503061),
                    Arthropod (n01767661), Reptile (n01661091),
                    Primate (n02469914), Fish (n02512053),
                    Feline (n02120997), Bovid (n02401031),
                    Amphibian (n01627424)\\
    		\hline  mixed-10  & Dog (n02084071), Bird (n01503061),
                    Insect (n02159955), Monkey (n02484322),
                    Car (n02958343), Cat (n02120997),
                    Truck (n04490091), Fruit (n13134947),
                    Fungus (n12992868), Boat (n02858304)\\		
    		\hline mixed-13  & Dog (n02084071), Bird (n01503061),
                    Insect (n02159955), Furniture (n03405725),
                    Fish (n02512053), Monkey (n02484322),
                    Car (n02958343), Cat (n02120997),
                    Truck (n04490091), Fruit (n13134947),
                    Fungus (n12992868), Boat (n02858304),
                    Computer (n03082979)\\		
    		\hline
    	\end{tabular}
	\end{center}
        \caption{ImageNet Superclass subsets}
        \label{tab:DataSetComp}
\end{table}




% Results

\subsection{Experiments and Analysis}
\label{sssec:clipAnalysis}
Given this setup we analyze the embeddings of the pre-trained CLIP Vision Transformers on the 2 data splits used to learn the parameters for the posterior distribution. For each network we compute the embeddings over all the datasets (train and test) shown in \autoref{tab:robustnessStatsImageNetSuperClasses} and use the training set to learn a linear classifier in order to quantify the linear separability of CLIP embeddings and also learn the parameters of the posterior to assess the quality of embeddings. We plot the data and network wise posterior ($\log$) probability and the linear classifier accuracy and show the pearson 
correlation ($\rho$) between the 2 quantities for each respective network in \autoref{fig:CLIPposteriorAnalysis}. \autoref{fig:netTrainDFs_CLIP} contain the results for the training set and the test set results are shown in \autoref{fig:netTestDFs_CLIP}.

\begin{figure}[!htb]
    \begin{center}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/Figures/netTrainDFs.pdf}
            \caption{Train Posterior and linear probe plots}
            \label{fig:netTrainDFs_CLIP}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/Figures/netTestDFs.pdf}
            \caption{Test Learned Posterior and linear probe plots}
            \label{fig:netTestDFs_CLIP}
        \end{subfigure}
        \begin{subfigure}{0.49\textwidth}
            \centering
            \includegraphics[width=\linewidth]{CLIPModelsBasic/Figures/netTestIndDFs.pdf}
            \caption{Test Independent Posterior and linear probe plots}
            \label{fig:netTestIndDFs_CLIP}
        \end{subfigure}
    \end{center}
    \caption{CLIP Embedding Posterior Analysis.}
    \label{fig:CLIPposteriorAnalysis}
\end{figure}



% Train Set Metrics

\begin{table}[!htb]
    % \begin{minipage}{0.5\textwidth}
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Training Set Metrics - ViT-B-16}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Train Log. Post. & -0.219 & -0.014 & -0.064 & -0.081 & -0.102 \\
            \hline
            Clustering Acc. Post. & 95.336 & 99.721 & 98.517 & 98.191 & 97.852\\
            \hline
            Linear Probe Acc. & 96.985 & 99.250 & 98.625 & 98.226 & 98.357\\
            \hline
        \end{tabular}
    \end{center}
    % \end{minipage}
    \caption{ViT-B-16 Train Posterior, clustering performance and linear probe statistics}
    \label{tab:trainingSetPerformanceCLIPvitb16}
\end{table}


\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Training Set Metrics - ViT-B-32}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Train Log. Post. & -0.271 & -0.020 & -0.109 & -0.112 & -0.137 \\
            \hline
            Clustering Acc. Post. & 94.209 & 99.595 & 97.471 & 97.477 & 97.105\\
            \hline
            Linear Probe Acc. & 95.700 & 98.729 & 97.254 & 97.407 & 97.538\\
            \hline
        \end{tabular}
    \end{center}
    \caption{ViT-B-32 Train Posterior, clustering performance and linear probe statistics}
    \label{tab:trainingSetPerformanceCLIPvitb32}
\end{table}



\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Training Set Metrics - ViT-L-14}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Train Log. Post. &  -0.125 & -0.001 & -0.012 & -0.022 & -0.029 \\
            \hline
            Clustering Acc. Post. & 97.356 & 99.975 & 99.732 & 99.512 & 99.388\\
            \hline
            Linear Probe Acc. & 97.604 & 99.691 & 99.440 & 98.978 & 98.962\\
            \hline
        \end{tabular}
    \end{center}
    \caption{ViT-L-14 Train Posterior, clustering performance and linear probe statistics}
    \label{tab:trainingSetPerformanceCLIPvitl14}
\end{table}


A more detailed presentation of results presented in \autoref{fig:netTrainDFs_CLIP} is shown in \autoref{tab:trainingSetPerformanceCLIPvitb16}, \autoref{tab:trainingSetPerformanceCLIPvitb32} and \autoref{tab:trainingSetPerformanceCLIPvitl14}. Further analyzing \autoref{fig:netTrainDFs_CLIP} for the training set we observe a strong correlation ($\rho$) between the $\log$ posterior probabilities and linear classifier accuracies. We also observe that for a given dataset a higher $\log$ posterior coincides with a higher linear classifier accuracy and a better clustering accuracy due to a higher posterior probability. We omitted the clustering accuracy plots for the posterior for brevity. But \autoref{tab:trainingSetPerformanceCLIPvitb16} - \autoref{tab:testIndSetPerformanceCLIPvitl14} contain those values. \\

% Test set metrics



\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Test Set Metrics - ViT-B-16}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Test Log. Post. & -0.265 & -0.225 & -0.133 & -0.168 & -0.186 \\
            \hline
            Clustering Acc. Post. & 94.319 & 95.500 & 96.947 & 96.300 & 96.131\\
            \hline
            Linear Probe Test Acc. & 97.143 & 99.125 & 98.279 & 98.200 & 98.411 \\
            \hline
        \end{tabular}
    \end{center}
    \caption{ViT-B-16 Test Posterior, clustering performance and linear probe statistics}
    \label{tab:testSetPerformanceCLIPvitb16}
\end{table}


\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Test Set Metrics - ViT-B-32}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Train Log. Post. &-0.313 & -0.254 & -0.200 & -0.207 & -0.225 \\
            \hline
            Clustering Acc. Post. & 93.294 & 94.938 & 95.420 & 95.433 & 95.311\\
            \hline
            Linear Probe Acc. & 94.494 & 97.688 & 97.197 & 97.833 & 97.771\\
            \hline
        \end{tabular}
    \end{center}
    \caption{ViT-B-32 Test Posterior, clustering performance and linear probe statistics}
    \label{tab:testSetPerformanceCLIPvitb32}
\end{table}



\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Test Set Metrics - ViT-L-14}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Train Log. Post. &  -0.172 & -0.180 & -0.064 & -0.082 & -0.112 \\
            \hline
            Clustering Acc. Post. & 96.335 & 96.438 & 98.557 & 98.167 & 97.643\\
            \hline
            Linear Probe Acc. & 97.943 & 99.375 & 99.223 & 99.100 & 99.154 \\
            \hline
        \end{tabular}
    \end{center}
    \caption{ViT-L-14 Test Posterior, clustering performance and linear probe statistics}
    \label{tab:testSetPerformanceCLIPvitl14}
\end{table}




% Test Set Ind Performance
Next, we continue the same analysis for \autoref{fig:netTestDFs_CLIP} of the test set and its accompanying metrics in \autoref{tab:testSetPerformanceCLIPvitb16}, \autoref{tab:testSetPerformanceCLIPvitb32} and \autoref{tab:testSetPerformanceCLIPvitl14}. The first observation that carries over from our previous analysis on the training set is that for a given dataset, networks with higher posterior also have better accuracies, however as shown in \autoref{fig:netTestDFs_CLIP} the correlation between those 2 sets of variables has reduced. Based on these observations we further investigate this by learning a posterior solely on the test data and comparing its generalization to the linear classifier and present the results in \autoref{fig:netTestIndDFs_CLIP} and the corresponding metrics in \autoref{tab:testIndSetPerformanceCLIPvitb16}, \autoref{tab:testIndSetPerformanceCLIPvitb32} and \autoref{tab:testIndSetPerformanceCLIPvitl14}. Paying close attention to performance of ViT-B-16 and ViT-B-32 on the big-12 dataset we observe that while ViT-B-16 has more linearly separable embeddings across the training and test as shown by better linear probe accuracy in comparison to ViT-B-32. The $\log$ posterior and therefore the corresponding clustering accuracy of ViT-B-32 is higher than ViT-B-16, this presents a counter example to the earlier analysis. Further, looking at ViT-B-32 and ViT-L-14 we observe that $\log$ posterior for both networks is the same for all the datasets but the linear probe performance of those embeddings have variations. This non dependence between linear probe values and  $\log$ posterior for perfectly clusterable data leads to an undefined Pearson Coefficient ($\rho$) as indicated by the value nan in \autoref{fig:netTestIndDFs_CLIP}.




\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Test (Ind.) Set Metrics - ViT-B-16}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Train Log. Post. & -0.0004 & 0.000 & 0.000 & 0.000 & 0.000 \\
            \hline
            Clustering Acc. Post. & 99.992 & 100.000 & 100.000 & 100.000 & 100.000\\
            \hline
            Linear Probe Acc. &97.143 & 99.125 & 98.279 & 98.200 & 98.411\\
            \hline
        \end{tabular}
    \end{center}
    \caption{ViT-B-16 Independently learned Test Posterior, its clustering performance and original linear probe statistics}
    \label{tab:testIndSetPerformanceCLIPvitb16}
\end{table}


\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Test (Ind.) Set Metrics - ViT-B-32}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Train Log. Post. & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
            \hline
            Clustering Acc. Post. & 100.000 & 100.000 & 100.000 & 100.000 & 100.000\\
            \hline
            Linear Probe Acc. & 94.494 & 97.688 & 97.197 & 97.833 & 97.771\\
            \hline
        \end{tabular}
    \end{center}
    \caption{ViT-B-32 Independently learned Test Posterior, its clustering performance and original linear probe statistics}
    \label{tab:testIndSetPerformanceCLIPvitb32}
\end{table}



\begin{table}[!htb]
    \begin{center}
        \begin{tabular}{ |c||c|c|c|c|c| }
            \hline
            \multicolumn{6}{|c|}{Test (Ind.) Set Metrics - ViT-L-14}\\
            \hline
            Datasets &  big-12 & geirhos-16 & living-9 & mixed-10 & mixed-13 \\
            \hline
            Train Log. Post. &  0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
            \hline
            Clustering Acc. Post. & 100.000 & 100.000 & 100.000 & 100.000 & 100.000\\
            \hline
            Linear Probe Acc. &  97.943 & 99.375 & 99.223 & 99.100 & 99.154 \\
            \hline
        \end{tabular}
    \end{center}
    \caption{ViT-L-14 Independently learned Test Posterior, its clustering performance and original linear probe statistics}
    \label{tab:testIndSetPerformanceCLIPvitl14}
\end{table}
















